Emergence of Tension Chains and Active Force Patterning

Viewed under a fluorescence microscope, the actomyosin cytoskeleton presents vivid streaks of lines together with persistent oscillatory waves. Using an active hydrodynamic approach, we show how a uniform distribution of single or mixture of contractile stresslets spontaneously segregate, followed by the formation of singular structures of high contractility (tension chains) in finite time. Simultaneously, the collection of stresslets exhibit travelling waves and swapping as a consequence of nonreciprocity. In the finite geometry of the cell, the collection of active tension chains can form an active web held together by specific anchoring at the cell boundary. On the other hand, preferential wetting at the cell boundary can reinforce active segregation in a mixture of stresslets leading to stratification.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
